An Efficient High-Order Meshless Method for Advection-Diffusion Equations on Time-Varying Irregular Domains

We present a high-order radial basis function finite difference (RBF-FD) framework for the solution of advection-diffusion equations on time-varying domains. Our framework is based on a generalization of the recently developed Overlapped RBF-FD method that utilizes a novel automatic procedure for computing RBF-FD weights on stencils in variable-sized regions around stencil centers. This procedure eliminates the overlap parameter $\delta$, thereby enabling tuning-free assembly of RBF-FD differentiation matrices on moving domains. In addition, our framework utilizes a simple and efficient procedure for updating differentiation matrices on moving domains tiled by node sets of time-varying cardinality. Finally, advection-diffusion in time-varying domains is handled through a combination of rapid node set modification, a new high-order semi-Lagrangian method that utilizes the new tuning-free overlapped RBF-FD method, and a high-order time-integration method. The resulting framework has no tuning parameters and has $O(N \log N)$ time complexity. We demonstrate high-orders of convergence for advection-diffusion equations on time-varying 2D and 3D domains for both small and large Peclet numbers. We also present timings that verify our complexity estimates. Finally, we utilize our method to solve a coupled 3D problem motivated by models of platelet aggregation and coagulation, once again demonstrating high-order convergence rates on a moving domain.

==> Overlap.tex <==
\section{An automatic overlapped RBF-FD method}
\label{sec:new_overlap}
We now present a generalization of the overlapped RBF-FD method that eliminates the overlap parameter $\delta$, and instead automatically computes, tests, and retains/discards candidate weights on a given stencil. Our approach for automation is to use two stability indicators to indicate whether a set of computed weights is of sufficient quality. In the discussion that follows, we will primarily focus on the stencil $P_1$, without loss of generality. In addition, we continue to use $\vy$ to refer to the point at which weights ${\bf w}^1(\vy)$ are computed, and $\vx$ to refer to points comprising the stencils, though these two are typically the same in practice.

\subsection{The local $\calL$-Lebesgue function}

As described in~\cite{ShankarJCP2017} and noted in~\cite{FlyerElliptic,Bayona2019}, local $\calL$-Lebesgue functions play a key role in assessing the suitability of a set of RBF-FD weights. Large values of the local $\calL$-Lebesgue function can lead to spurious eigenvalues in the differentiation matrix corresponding to $\calL$. This fact was used to develop a stability indicator for the overlapped RBF-FD method in~\cite{ShankarJCP2017} which was used to discard unsuitable weights on a given stencil. Recall that $\vx_{\calI^1_1}$ and its $n-1$ neighbors form the stencil $P_1$. Then, letting $\vy_1 = \vx_{\calI^1_1}$, one can define the $\calL$-Lebesgue function at $\vx_1$ as the $\ell_1$-norm of the weight vector at that point:
\begin{align}
\Lambda_{\calL}(\vy_1) = \|{\bf w}^1(\vy_1)\|_1.
\end{align}
Let $\mathbb{B}_{11}'$ (analogous to $\mathbb{B}_1$ from the previous section) be the set of points $\vy \in P_1$ at which valid RBF-FD weights are available. This set can be defined as:
\begin{align}
\mathbb{B}_{11}' = \{\vy \in P_1 \mid \Lambda_{\calL}(\vy) \leq \Lambda_{\calL}(\vy_1) \},
\label{eq:leb_set}
\end{align}
\emph{i.e.}, the set of all points in $P_1$ where the $\calL$-Lebesgue function takes on values smaller than at the stencil center $\vy_1$. In~\cite{ShankarJCP2017}, the RBF-FD weights from lower-order methods were computed by solving \eqref{eq:rbf_linsys} (with the right hand side determined by the overlap parameter), but were tested (and if necessary, discarded) using the $\calL$-Lebesgue stability indicator before assembly into the corresponding differentiation matrix in Step 12 of Algorithm \ref{alg:old_assembly}. In this work, we do not use the overlap parameter, but instead directly compute RBF-FD weights for every $\vy \in P_1$, and assess their suitability using the $\calL$-Lebesgue function at that point. This process is repeated on every stencil.

\subsection{An oscillation indicator for ${\bf w}^1$}

The family of interpolants $s_1(\vx,\vy)$ is defined by the family of RBF-FD weights $w^1_j(\vy), j=1,\ldots,n$ and polynomial weights $\lambda^1_i(\vy),i=1,\ldots,M$; here, each specific value of $\vy \in P_1$ results in a different set of RBF-FD and polynomial weights, though the RBF and polynomial bases themselves are fixed. All RBFs have an associated reproducing kernel Hilbert space called the native space~\cite{Fasshauer:2007}. The \emph{native space semi-norm} of an RBF interpolant formed from PHS RBF is a measure of how much the interpolant oscillates~\cite{iske:2002}. In the standard interpolation setting (rather than the RBF-FD setting), PHS RBF interpolants with RBF interpolation matrix $A$ and RBF coefficient vector $\vc$ have a native space semi-norm of $|\vc^T A \vc|$~\cite{iske:2002}. However, in the RBF-FD context on the stencil $P_1$, it is not straightforward to define an analogous norm involving the weights. Nevertheless, we can define an analogous oscillation indicator for the weights used in $s_1(\vx,\vy)$ as:
\begin{align}
\mathcal{S}\lf(\lf.s_1(\vx,\vy)\rt|_{\vx,\vy \in P_1}\rt) = 
\lf|
\begin{bmatrix} W_1^T & \lf(W^{\psi}_1\rt)^T \end{bmatrix}
\begin{bmatrix}
A_1 & \Psi_1 \\
\Psi_1^T & O
\end{bmatrix}
\begin{bmatrix}
W_1 \\
W^{\psi}_1
\end{bmatrix}\rt|.
\end{align}
While this quantity can be further simplified, the above form is perfectly amenable to computation. More importantly, it serves as a second stability indicator for the overlapped RBF-FD method. We use it to define a set $\mathbb{B}_{12}$ (analogous to $\mathbb{B}_{11}$):
\begin{align}
\mathbb{B}_{12}' = \{\vy \in P_1 \mid \mathcal{S}\lf(\lf.s_1(\vx,\vy)\rt|_{\vx,\vy \in P_1}\rt)  \leq \mathcal{S}\lf(\lf.s_1(\vx,\vy_1)\rt|_{\vx \in P_1}\rt) \}.
\label{eq:ns_set}
\end{align}
While~\cite{ShankarJCP2017} found that the $\calL$-Lebesgue indicator is sufficient for low-order methods, we found that the above oscillation indicator is the better indicator for high-order ones as it appears to measure the amount of oscillation induced by the RBF-FD weights on derivatives. While theoretical justification for this indicator is lacking, our experiments indicate that this indicator works well in conjunction with the $\calL$-Lebesgue indicator.

\subsection{Parameter-Free Assembly}
Once both stability indicators are used to define the sets $\mathbb{B}_{11}$ and $\mathbb{B}_{12}$, we can now define a single set $\mathbb{B}_1'$ of points whose weights are acceptable from the stencil $P_1$ as:
\begin{align}
\mathbb{B}_1' = \mathbb{B}_{11} \cap \mathbb{B}_{12},
\label{eq:final_seta}
\end{align}
\emph{i.e.}, the set of nodes for which we deem the RBF-FD weights as suitable is the intersection of the sets of nodes which pass both stability indicator tests. In general, for the stencil $P_k$, we have 
\begin{align}
\mathbb{B}_k' = \mathbb{B}_{k1} \cap \mathbb{B}_{k2}.
\label{eq:final_setb}
\end{align}
It is also useful to obtain the global indices of the points each ball $\mathbb{B}_k'$:
\begin{align}
R_k' = \{\calR_1^k, \calR_2^k, \ldots, \calR_{p_k}^k\},
\label{eq:final_indset}
\end{align}
where $p_k = |\mathbb{B}_k'|$.
Note that with the definition of the sets $\mathbb{B}_k'$, the stencil centers $\vy_k = \vx_{\calI^k_1}$ will automatically pass our stability tests, and an assembly algorithm based on the stencil centers is guaranteed to converge in that every point $\vx \in X$ is guaranteed to receive a set of RBF-FD weights. 

In practice, even for irregular nodes, we find that the number of stencils $N_s$ can be much smaller than the number of nodes $N$. In addition, we find that the order $\theta$ of the differential operator $\calL$ can influence the number of stencils, with higher-order operators leading to fewer stencils. This is likely due to the fact that our formula for the stencil size $n$ depends indirectly on $\theta$, and also due to the fact that larger stencils result in better behaved RBF-FD weights~\cite{ShankarJCP2017}. 

The full process for assembling the sparse differentiation matrix using the indicators \eqref{eq:leb_set} and \eqref{eq:ns_set} is described in Algrothm \ref{alg:new_assembly}. The new algorithm no longer requires an overlap parameter, and is therefore much more robust to irregularities in node sets. More importantly, if the node sets are changing in time (as they do in the present study), this approach obviates the need for hand-tuning.
\begin{algorithm}
\caption{Automatic Differentiation matrix assembly}
\label{alg:new_assembly}
\begin{algorithmic}[1]	
  \Statex{\bf Given}: $X = \{\vx_k\}_{k=1}^N$, the set of nodes in the domain.	
	\Statex{\bf Given}: $\calL$, the linear differential operator to be approximated.
	\Statex{\bf Given}: $n << N$, the stencil size.
	\Statex{\bf Generate}: $L$, the $N \times N$ differentiation matrix approximating $\calL$ on the set $X$.	
	\Statex{\bf Generate}: $N_s$, the number of stencils.
	\State Build a k-d tree on the set $X$ in $O(N \log N)$ operations.
	\State Initialize $g$, an array of $N$ flags set to 0.
	\State Initialize the stencil counter, $N_{s}=0$.
	\For {$k=1,N$}
		\If {$g(k)$ == 0}		
				\State Use k-d tree to determine $\{\vx_{\calI^k_1},\hdots,\vx_{\calI^k_n}\}$. Here, $\calI^k_1 = k$.
				\State Use \eqref{eq:rbf_linsys} to compute $W_k$, the $n \times n$ matrix of RBF-FD weights on the full stencil $P_1$.
				\State Find the set $\mathbb{B}_k'$ using \eqref{eq:leb_set},\eqref{eq:ns_set}, and \eqref{eq:final_setb}.
				\State Also find the set $R_k'$ as defined in \eqref{eq:final_indset} by keeping track of global indices of elements of $\mathbb{B}_k'$.
				\For {$i=1,n$}
					\If {$\vx_{\calR^k_i} \notin \mathbb{B}_k'$}
							\State CONTINUE.
					\EndIf
					\State Set $g\lf(\calR^k_i\rt) = 1$.					
					\For{$j=1,n$}
							\State Set $L\lf(\calR^k_i,\calI^k_j\rt) = W_k(j,i)$.
					\EndFor
				\EndFor				
		\EndIf
	\EndFor
\end{algorithmic}
\end{algorithm}


==> RBFReview.tex <==
\section{A review of overlapped RBF-FD}
\label{sec:old_overlap}

We now present a description of the overlapped RBF-FD method~\cite{ShankarJCP2017,SFJCP2018,SNKJCP2018}. Let $X = \{\vx_k\}_{k=1}^N$ be a global set of nodes on a domain $\Omega \subset \mathbb{R}^d$. Define the stencil $P_k$ to be the set of nodes containing node $\vx_{\calI^k_1}$ and its $n-1$ nearest neighbors $\{\vx_{\calI^k_2},\hdots,\vx_{\calI^k_n}\}$; here, $\{\calI^k_1,\hdots,\calI^k_n\}$ are indices that map into the global node set $X$. Without loss of generality, we focus on the stencil $P_1$. First, define the stencil width $\rho_1$ as
%
\begin{align}
\rho_1 = \max\limits_{1 \leq j \leq n} \|\vx_{\calI^1_1} - \vx_{\calI^1_j}\|,
\label{eq:stencil_rad}
\end{align}
%
and an \emph{overlap parameter} $\delta \in (0,1]$. Let define $R_1$ be the set of global indices of the $p_1$ nodes in the stencil $P_1$ that are within the distance $(1-\delta)\rho_1$ from $\vx_{\calI^1_1}$. This can be written as
\begin{align}
R_1 = \{\calR^1_1, \calR^1_2, \hdots, \calR^1_{p_1}\}.
\label{eq:ball_inds}
\end{align}
Next, let $\mathbb{B}_1$ be the ball containing the nodes whose indices are in $R_1$. Thus, 
\begin{align}
\mathbb{B}_1 = \{\vx_{\calR^1_1}, \hdots, \vx_{\calR^1_{p_1}} \}.
\label{eq:ball_pts}
\end{align}
The overlapped RBF-FD method involves computing RBF-FD weights for all the nodes in the ball $\mathbb{B}_1$ (defined by $\delta$). 

The weights for all the nodes in $\mathbb{B}_1$ with indices in $R_1$ are computed using the following augmented local RBF interpolant on $P_1$:
\begin{align}
s_1(\vx,\vy) = \sum\limits_{j=1}^n w^1_j(\vy) \|\vx - \vx_{\calI^1_j}\|^m + \sum\limits_{i=1}^{M} \lambda^1_i(\vy) \psi^1_i(\vx),
\label{eq:rbf_interp}
\end{align}
where $\|\vx - \vx_{\calI^1_j}\|^m$ is the polyharmonic spline (PHS) RBF of degree $m$ ($m$ is odd), and $\{\psi^1_i(\vx)\}$ form a basis for the space of polynomials of total degree degree $\ell$ in $d$ dimensions, which gives $M = {\ell + d \choose d}$; common choices for these include monomials~\cite{SFJCP2018} or orthogonal polynomials~\cite{SNKJCP2018}. In this work, we select the $\psi^1_i(\vx)$ functions to be Legendre polynomials. The $n$ overlapped RBF-FD weights associated with the point $\vy$ are $w^1_j(\vy), j=1,\hdots,n$. We compute the weights for the linear operator $\calL$ uniquely at all nodes in $\mathbb{B}_1$ with indices in the set $R_1$ by imposing the following two (sets of) conditions:
\begin{align}
\lf.s_1 \rt|_{\vx \in P_1, \vy \in \mathbb{B}_1} &= \lf.\calL \|\vx - \vx_{\calI^1_j}\|^m\rt|_{\vx \in \mathbb{B}_1}, j=1,\hdots,n, \label{eq:interp_constraint}\\
\sum_{j=1}^n \lf.w_j^1(\vy) \psi_i^1(\vx) \rt|_{\vx \in P_1, \vy \in \mathbb{B}_1} &= \lf.\calL \psi^1_i(\vx)\rt|_{\vx \in \mathbb{B}_1}, i=1,\hdots,M. \label{eq:poly_constraint}
\end{align}
These conditions enforce that the weights are exact for both $\calL$ applied to the PHS RBF and to the polynomial basis. In practice, $n = 2M+1$~\cite{ShankarJCP2017,SFJCP2018,FlyerNS,FlyerPHS}. The constraints \eqref{eq:interp_constraint}--\eqref{eq:poly_constraint} for determining the weights in \eqref{eq:rbf_interp} can be collected into the following block linear system:
\begin{align}
\begin{bmatrix}
A_1 & \Psi_1 \\
\Psi_1^T & 0
\end{bmatrix}
\begin{bmatrix}
W_1 \\
W^{\psi}_1
\end{bmatrix}
=
\begin{bmatrix}
B_{A_1} \\
B_{\Psi_1}
\end{bmatrix},
\label{eq:rbf_linsys}
\end{align}
where
\begin{align}
(A_1)_{ij} &= \|\vx_{\calI^1_i} - \vx_{\calI^1_j} \|^m, i,j=1,\hdots,n, \\
(\Psi_1)_{ij} &= \psi^1_j(\vx_{\calI^1_i}), i=1,\hdots,n, j=1,\hdots,M,\\
(B_{A_1})_{ij} &= \lf.\calL \|\vx - \vx_{\calI^1_i} \|^m \rt|_{\vx = \vx_{\calR^1_j}}, i=1,\hdots,n, j=1,\hdots,p_1, \\
(B_{\Psi_1})_{ij} &= \lf.\calL \psi^1_i(\vx)\rt|_{\vx = \vx_{\calR^1_j}}, i=1,\hdots,M, j=1,\hdots,p_1.
\end{align}
$W_1$ is the matrix of overlapped RBF-FD weights, with each column containing the RBF-FD weights for a point $\vx \in \mathbb{B}_1$. 

The linear system \eqref{eq:rbf_linsys} has a unique solution if the nodes in $P_1$ are distinct and $\Psi_1$ has full column rank~\cite{Fasshauer:2007,Wendland:2004}. The matrix of polynomial coefficients $W^{\psi}_1$ enforces the polynomial reproduction constraint \eqref{eq:poly_constraint}; in the case of RBF-FD, this serves as a set of Lagrange multipliers. This constraint ensures that the \emph{local} approximation error is bounded by $O \lf(h^{\ell+1-\theta} \rt)$, where $\theta$ is the order of the differential operator $\calL$, and $h$ is the largest distance between the point at which the weights are computed and every other point in the stencil~\cite{DavydovSchaback2018}. 

The RBF-FD weights for every stencil $P_j$ in the domain can be assembled into an $N\times N$ sparse differentiation matrix, with each stencil weight matrix $W_1$ populating $p_1$ rows of the differentiation matrix at once. This assembly (as described in~\cite{SFJCP2018}) is presented in Algorithm \ref{alg:old_assembly} for completeness.
\begin{algorithm}
\caption{Differentiation matrix assembly using an overlap parameter $\delta$}
\label{alg:old_assembly}
\begin{algorithmic}[1]	
  \Statex{\bf Given}: $X = \{\vx_k\}_{k=1}^N$, the set of nodes in the domain.
	\Statex{\bf Given}: $\delta \in (0,1]$, the overlap parameter.
	\Statex{\bf Given}: $\calL$, the linear differential operator to be approximated.
	\Statex{\bf Given}: $n$, the stencil size.
	\Statex{\bf Generate}: $L$, the $N \times N$ differentiation matrix approximating $\calL$ on the set $X$.
	\Statex{\bf Generate}: $N_s$, the number of unique stencils.
	\State Build a k-d tree on the set $X$ in $O(N \log N)$ operations.
	\State Initialize $g$, an array of flags set 0.
	\State Initialize the stencil counter, $N_s=0$.
	\For {$k=1,N$}
		\If {$g(k)$ == 0}		
				\State Use k-d tree to get $\{\vx_{\calI^k_1},\hdots,\vx_{\calI^k_n}\}$. Here, $\calI^k_1 = k$.
				\State Get $R_k = \{\calR^k_1, \hdots, \calR^k_{p_k}\}$ and $\mathbb{B}_k = \{\vx_{\calR^k_1}, \hdots, \vx_{\calR^k_{p_k}} \}$ using \eqref{eq:stencil_rad}--\eqref{eq:ball_pts}.
				\State Use \eqref{eq:rbf_linsys} to compute $W_k$, the $n \times p_k$ matrix of RBF-FD weights.
				\For {$i=1,p_k$}
					\State Set $g\lf(\calR^k_i\rt) = 1$.	
					\For{$j=1,n$}
							\State Set $L\lf(\calR^k_i,\calI^k_j\rt) = W_k(j,i)$.
					\EndFor
				\EndFor
				\State Set $N_s = N_s+1$.
		\EndIf
	\EndFor
\end{algorithmic}
\end{algorithm}

A drawback with the overlapped RBF-FD approach is that poor choices of $\delta$ (close to 0) could result in spurious eigenvalues in the differentiation matrix for $\calL$. While recipes for $\delta$ have been provided~\cite{ShankarJCP2017,SFJCP2018,SNKJCP2018}, these were ad-hoc choices without much theoretical justification. In the next section, we describe a new algorithm for weight computation and differentiation matrix assembly that completely does away with the overlap parameter.

==> Stability.tex <==
\section{A new scaling law for $m$ and $\ell$}
\label{sec:stab}

The selection of the degree $m$ of the PHS RBF requires more thought. On the one hand, $m$ is known to control the constant in the RBF-FD error estimate \eqref{eq:error_estimate}, with higher values of $m$ giving lower errors~\cite{FlyerPHS,BarnettPHS}. On the other hand, larger values of $m$ may cause greater instability, as the smallest eigenvalue of the block matrix from \eqref{eq:rbf_linsys} can be bounded from below by $q^m$, where $q$ is the separation distance of the stencil $P_1$; see~\cite{Wendland:2004} for some preliminary estimates, and~\cite{FlyerNS} for remarks about stability. A third more subtle issue is the question of whether $m$ and $\ell$ should be related. Historically, it was common to use the \emph{classical scaling law}~\cite{iske2002}:
\begin{align}
m = 2\ell+1,
\label{eq:scaling_law_classical}
\end{align}
where $\ell$ is selected to be the minimum to prove unisolvency for the RBF interpolant with $\phi(r) = r^m$. This approach was also recently used for PHS-based methods for advection on the sphere~\cite{ShankarWrightJCP2017}, and advection and reaction-diffusion equations on more general manifolds~\cite{SNKJCP2018}. However, modern PHS RBF-FD methods for Euclidean domains decouple $m$ and $\ell$~\cite{FlyerNS,FlyerPHS,BarnettPHS,ShankarJCP2017}. Our goal is to attempt to find a scaling law that produces the smallest spurious eigenvalue (if any) in the spectrum of the discrete Laplacian $L$. To that end, we explored two alternatives to the classical scaling law. The first alternative is:
\begin{align}
m = 
\begin{cases}
	\hfill \ell \hfill & \text{if $\ell$ is odd} \\
	\hfill \ell+1 \hfill & \text{if $\ell$ is even}\\
\end{cases}
\label{eq:scaling_law_1}
\end{align}
which serves to gently increase $m$ as $\ell$ is increased. The second alternative, which we ultimately settled on, is:
\begin{align}
m = 
\begin{cases}
	\hfill \ell \hfill & \text{if $\ell$ is odd} \\
	\hfill \ell-1 \hfill & \text{if $\ell$ is even}\\
\end{cases}
\label{eq:scaling_law_2}
\end{align}
The eigenvalues for the discrete Laplacian $L$ computed using the classical scaling law, these two alternatives, and the choice of $m=3$ are shown for $N=658$ nodes on the disk using $\ell=6$ in Figure \ref{fig:eigs_laws1}.
\begin{figure}[h!]
\centering
\subfloat[$m=2\ell+1$]
{
	\includegraphics[scale=0.6]{"Figures/Eig2lp1".png}
	\label{fig:c11}	
}
\subfloat[$m=\ell+1$]
{
	\includegraphics[scale=0.6]{"Figures/Eig7".png}
	\label{fig:c12}	
}

\subfloat[$m = \ell-1$]
{
	\includegraphics[scale=0.6]{"Figures/Eiglm1".png}
	\label{fig:c21}	
}
\subfloat[$m = 3$]
{
	\includegraphics[scale=0.6]{"Figures/Eig3".png}
	\label{fig:c22}	
}
\caption{Spectrum of the discrete Laplacian $L$ on a node set with $N=658$ nodes for different relationships between $m$ and $\ell$. The node set here was a set of Poisson disk samples generated on the disk using the method from~\cite{SFKSISC2017}.}
\label{fig:eigs_laws1}
\end{figure}
From Figure \ref{fig:c11}, it is clear that the classical scaling law $m=2\ell+1$ results in a large spurious eigenvalue. In general, all the other scaling laws appear to give very similar results, albeit with some subtle differences. Figure \ref{fig:c12} uses the scaling law $m=\ell+1$, while Figure \ref{fig:c21} uses the scaling law $m = \ell-1$; clearly, both produce almost identical results, with the exception that $m=\ell+1$ results in a slightly larger spurious eigenvalue. Continuing this trend, it may be tempting to always simply choose a very small reasonable value of $m$. However, Figure \ref{fig:c22} with $m=3$ shows that this may not be entirely advisable either, since the largest spurious eigenvalue here is actually larger than the cases of $m=\ell+1$ and $m=\ell-1$. 
\begin{figure}[h!]
\centering
\subfloat[$m=2\ell+1$]
{
	\includegraphics[scale=0.6]{"Figures/Eig2lp1_2".png}
	\label{fig:d11}	
}
\subfloat[$m=\ell+1$]
{
	\includegraphics[scale=0.6]{"Figures/Eiglp1_2".png}
	\label{fig:d12}	
}

\subfloat[$m = \ell-1$]
{
	\includegraphics[scale=0.6]{"Figures/Eiglm1_2".png}
	\label{fig:d21}	
}
\subfloat[$m = 3$]
{
	\includegraphics[scale=0.6]{"Figures/Eig3_2".png}
	\label{fig:d22}	
}
\caption{Spectrum of the discrete Laplacian $L$ on a node set with $N=919$ nodes for different relationships between $m$ and $\ell$. The node set here was a set of Poisson disk samples generated on the disk using the method from~\cite{SFKSISC2017}.}
\label{fig:eigs_laws2}
\end{figure}
The spectrum of $L$ for different scaling laws for $N=919$ nodes with $\ell=6$ is shown in Figure \ref{fig:eigs_laws2}. Once again, $m=2\ell+1$ can be rejected as extremely unstable, even after refinement (Figure \ref{fig:d11}). However, the gaps between the other scaling laws have widened slightly as well. For instance, $m=\ell+1$ (Figure \ref{fig:d12}) now results in a spurious eigenvalue that is twice as large as $m=\ell-1$ (Figure \ref{fig:d21}). Even more interestingly, $m=3$ (Figure \ref{fig:d22}) results in a spurious eigenvalue whose real part is much larger than the $m=\ell+1$ and $m=\ell-1$ cases. Once again, the most stable choice appears to be $m = \ell-1$. Picking a fixed value of $m=3$ (or any other number) regardless of the choice of $\ell$ may be inadvisable on Euclidean domains except when the node sets are very regular. These trends continue for different values of $\ell$ (not shown). It may be the case that the correct scaling relationship needs to be reevaluated for each type of node set used.

Thus far, we have only discussed the \emph{global} stability associated with the different scaling laws. It is reasonable to expect that these global patterns are reflected in some way at the stencil level. In other words, we expect that the global stability must be connected to \emph{local} stability in some way.  Before we can explore this connection, we must first define a few quantities. Returning to the stencil $P_1$, consider the \emph{local $\calL$-Lebesgue function} of the augmented RBF interpolant $s_1(\vx,\vy)$ used for approximating the operator $\calL$, defined as
\begin{align}
\Lambda^1_{\calL}(\vy) = \sum\limits_{j=1}^n |w^1_j(\vy)| = \|{\bf w}^1\|_1,
\end{align}
that is, the 1-norm of the RBF-FD weight vector at a point. Let $w^1_1(\vy)$ be the RBF-FD weight associated with the stencil point $\vy$. From~\cite{ShankarJCP2017}, we have the sufficient condition for all eigenvalues of the differentiation matrix $L$ (corresponding to $\calL$) having non-positive real parts as:
\begin{align}
2w^1_1(\vy) \geq - \Lambda^1_{\calL}(\vy).
\end{align}
This condition highlights the connection between the local Lebesgue function (itself connected to the stability of the local RBF interpolant~\cite{Wendland:2004}) and the \emph{global} stability of the RBF-FD method. In general, large values of $\Lambda^1_{\calL}(\vy)$ are associated with instability, and typically produce spurious eigenvalues with positive real parts~\cite{ShankarJCP2017}. To examine the impact of the scaling laws \eqref{eq:scaling_law_classical}--\eqref{eq:scaling_law_2} on the local Lebesgue functions (and therefore local stability), we will now study the local $\Delta$-Lebesgue functions for a set of $N = 4000$ Halton points in $[-1,1]^2$, where $\Delta$ is the Laplacian; evenly-spaced points are used on the boundary; these Halton points are typically even more scattered than Poisson disk samples, and represent a worst-case scenario. The results are shown in Figure \ref{fig:leb_c1}.
\begin{figure}[h!]
\centering
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_9_4".pdf}
	\label{fig:leb_c13}	
}
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_5_4".pdf}
	\label{fig:leb_c11}	
}
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_3_4".pdf}
	\label{fig:leb_c12}	
}

\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_13_6".pdf}
	\label{fig:leb_c23}	
}
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_7_6".pdf}
	\label{fig:leb_c21}	
}
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_5_6".pdf}
	\label{fig:leb_c22}	
}

\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_17_8".pdf}
	\label{fig:leb_c33}	
}
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_9_8".pdf}
	\label{fig:leb_c31}	
}
\subfloat[]
{
	\includegraphics[scale=0.4]{"Figures/LocalStab_7_8".pdf}
	\label{fig:leb_c32}	
}
\caption{Local $\Delta$-Lebesgue functions for different scaling laws on a logarthmic scale. The figure contrasts \eqref{eq:scaling_law_classical} (left), \eqref{eq:scaling_law_1} (middle), and \eqref{eq:scaling_law_2} (right). Lighter colors indicate larger values, which in turn indicate greater potential for instability.}
\label{fig:leb_c1}
\end{figure}
The first column in Figure \ref{fig:leb_c1} corresponds to the classical law \eqref{eq:scaling_law_classical}, the second to \eqref{eq:scaling_law_1}, and the third to \eqref{eq:scaling_law_2}. The colorbar scale is fixed across each row, but allowed to increase between rows to make clear that RBF-FD weights can increase in magnitude as the polynomial degree is increased. Immediately, it is clear that the classical scaling law results in the largest weights, and is consequently almost always unstable (Figures \ref{fig:leb_c13},\ref{fig:leb_c23}, \ref{fig:leb_c33}).  Careful observation also shows that the last column (corresponding to \eqref{eq:scaling_law_2}) results in more stable approximations than the middle column (corresponding to \eqref{eq:scaling_law_1}), which matches our conclusions from the eigenvalue plots (Figures \ref{fig:eigs_laws1} and \ref{fig:eigs_laws2}). In general, we find that the scaling law \eqref{eq:scaling_law_2} produces stable approximations across a wide range of parameters, and therefore we use it in this article.

%\begin{figure}[h!]
%\centering
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabFlyer33".pdf}
	%\label{fig:leb_c1a}	
%}
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabNew33".pdf}
	%\label{fig:leb_c1b}	
%}
%
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabFlyer45".pdf}
	%\label{fig:leb_c1c}	
%}
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabNew45".pdf}
	%\label{fig:leb_c1d}	
%}
%
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabFlyer94".pdf}
	%\label{fig:leb_c1e}	
%}
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabNew94".pdf}
	%\label{fig:leb_c1f}	
%}
%\caption{Local $\Delta$-Lebesgue functions for different scaling laws on a logarthmic scale. $m=7$ is used for the modern scaling law (left column), while \eqref{eq:scaling_law} is used for the right column. Lighter colors indicate larger values, which in turn indicate greater potential for instability.}
%\label{fig:leb_c1}
%\end{figure}
%We remind the reader that there are three such relationships to be examined:
%\begin{enumerate}
%\item The classical law: $m = 2\ell + 1$.
%\item The modern law: fixed $m$, regardless of $\ell$. Flyer et al~\cite{FlyerNS} pick $m=3$ and $m=7$, with a passing remark on the improved stability of the former over the latter.
%\item Our new law \eqref{eq:scaling_law}: $m = \ell + 1$ if $\ell$ is even, $m = \ell$ if $\ell$ is odd.
%\end{enumerate}
%Before proceeding, we remark that the error estimate \eqref{eq:error_estimate} shows that convergence \emph{rates} are not affected by the choice of $m$. However, the growth function $P(\vx)$ in that estimate controls both the error constant and the stability of the interpolation process~\cite{DavydovMinimal2016}. Indeed, Flyer et al showed that larger values of $m$ can lead to greater accuracy~\cite{FlyerPHS}.
%\begin{figure}[h!]
%\centering
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabFlyer76".pdf}
	%\label{fig:leb_c2a}	
%}
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabNew76".pdf}
	%\label{fig:leb_c2b}	
%}
%
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabFlyer114".pdf}
	%\label{fig:leb_c2c}	
%}
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabNew114".pdf}
	%\label{fig:leb_c2d}	
%}
%
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabFlyer187".pdf}
	%\label{fig:leb_c2e}	
%}
%\subfloat[]
%{
	%\includegraphics[scale=0.5]{"Figures/LocalStabNew187".pdf}
	%\label{fig:leb_c2f}	
%}
%\caption{Local $\Delta$-Lebesgue functions for different scaling laws on a logarthmic scale. $m=11$ is used for the modern scaling law (left column), while \eqref{eq:scaling_law} is used for the right column. Lighter colors indicate larger values, which in turn indicate greater potential for instability.}
%\label{fig:leb_c2}
%\end{figure}
%To examine the impact of these scaling laws on stability, we will focus on the local $\Delta$-Lebesgue functions for a set of Halton points in $[-1,1]^2$, where $\Delta$ is the Laplacian; evenly-spaced points are used on the boundary. We use the fixed value $m=7$ for the modern law, increase the polynomial degree $\ell$, and plot a few of the resulting $\Delta$-Lebesgue functions. The results for the modern law and our proposed new law are shown in Figure \ref{fig:leb_c1} for $\ell = 4,5,8$ ($\ell = 6,7$ are omitted for as both approximations are identical for these cases). As one goes down the figure columns (Figures \ref{fig:leb_c1a}--\ref{fig:leb_c1d}), it appears that our new scaling law from \eqref{eq:scaling_law} results in more stable approximations until $\ell>7$, at which point the modern law with $m=7$ suddenly results in a more stable approximation (Figures \ref{fig:leb_c1e} shows better results than \ref{fig:leb_c1f}). We also repeat the above experiment using $m=11$ for the modern law to show that the pattern from Figure \ref{fig:leb_c1} persists. The results are shown in Figure \ref{fig:leb_c2}. The choice of $m=11$ results in a more stable approximation when $\ell\geq 11$.
%
%In this article, we restrict ourselves to methods with polynomial degree $\ell \in [3,7]$, which results in second to sixth order methods. For this regime, our proposed scaling law \eqref{eq:scaling_law} is perfectly adequate. However, in general, it is clear that a PHS RBF $r^m$ produces the most stable approximation for a specific range for $\ell$, given by $\ell \in [m,m+1]$. In other words, given a polynomial degree $\ell$, the most stable RBF-FD approximation is produced by the PHS RBF $r^m$, where $m \leq \ell$ is the closest odd number to $\ell$. To the best of our knowledge, this pattern has never been reported in the literature.
